Osmotic buckling of spherical capsules

We study the buckling of elastic spherical shells under osmotic pressure with the osmolyte concentration of the exterior solution as control parameter. We compare our results for the bifurcation behavior with results for buckling under mechanical pressure control, that is, with an empty capsule interior. We find striking differences for the buckling states between osmotic and mechanical buckling. Mechanical pressure control always leads to fully collapsed states with opposite sides in contact, whereas uncollapsed states with a single finite dimple are generic for osmotic pressure control. For sufficiently large interior osmolyte concentrations, osmotic pressure control is qualititatively similar to buckling under volume control with the volume prescribed by the osmolyte concentrations inside and outside the shell. We present a quantitative theory which also captures the influence of shell elasticity on the relation between osmotic pressure and volume. These findings are relevant for the control of buckled shapes in applications. We show how the osmolyte concentration can be used to control the volume of buckled shells. An accurate analytic formula is derived for the relation between the osmotic pressure, the elastic moduli and the volume of buckled capsules. This also allows to use elastic capsules as osmotic pressure sensors or to deduce elastic properties and the internal osmolyte concentration from shape changes in response to osmotic pressure changes. We apply our findings to published experimental data on polyelectrolyte capsules.

==> def_derivatives.tex <==
% Ableitung
\makeatletter
\newcommand\der[2]{%
    \begingroup
    \@temptokena{\@gobble}%
    \@tempcnta\z@
    \@for\var:=#2\do{%
        \expandafter\@der\var\relax
    }%
    \ensuremath{\frac{\diff
    \ifnum\@tempcnta>\@ne
        ^{\the\@tempcnta}%
    \fi
    #1}{\the\@temptokena}}%
    \endgroup
}
\def\@der#1#2\relax{%
    \ifx\relax#2\relax
        \advance\@tempcnta by \@ne
        \@temptokena\expandafter{\the\@temptokena\null\diff{#1}}%
    \else
	\if!\ifnum9<1#2!\else_\fi%falls #2 eine Zahl ist...
	  \advance\@tempcnta by #2\relax
	  \@temptokena\expandafter{\the\@temptokena\null\diff{#1}^{#2}}%
	\else
	  \advance\@tempcnta by \@ne
	  \@temptokena\expandafter{\the\@temptokena\null\diff#1#2}
	\fi
    \fi
}
\makeatother

% Ableitung flacher Bruch
\makeatletter
\newcommand\fder[2]{%
    \begingroup
    \@temptokena{\@gobble}%
    \@tempcnta\z@
    \@for\var:=#2\do{%
        \expandafter\@fder\var\relax
    }%
    \ensuremath{{\diff
    \ifnum\@tempcnta>\@ne
        ^{\the\@tempcnta}%
    \fi
    #1}/{\the\@temptokena}}%
    \endgroup
}
\def\@fder#1#2\relax{%
    \ifx\relax#2\relax
        \advance\@tempcnta by \@ne
        \@temptokena\expandafter{\the\@temptokena\null\diff{#1}}%
    \else
	\if!\ifnum9<1#2!\else_\fi%falls #2 eine Zahl ist...
	  \advance\@tempcnta by #2\relax
	  \@temptokena\expandafter{\the\@temptokena\null\diff{#1}^{#2}}%
	\else
	  \advance\@tempcnta by \@ne
	  \@temptokena\expandafter{\the\@temptokena\null\diff#1#2}
	\fi
    \fi
}
\makeatother

% partielle Ableitung
\makeatletter
\newcommand\pder[2]{%
    \begingroup
    \@temptokena{\@gobble}%
    \@tempcnta\z@
    \@for\var:=#2\do{%
        \expandafter\@pder\var\relax
    }%
    \ensuremath{\frac{\partial
    \ifnum\@tempcnta>\@ne
        ^{\the\@tempcnta}%
    \fi
    #1}{\the\@temptokena}}%
    \endgroup
}
\def\@pder#1#2\relax{%
    \ifx\relax#2\relax
        \advance\@tempcnta by \@ne
        \@temptokena\expandafter{\the\@temptokena\null\partial{#1}}%
    \else
	\if!\ifnum9<1#2!\else_\fi%falls #2 eine Zahl ist...
	  \advance\@tempcnta by #2\relax
	  \@temptokena\expandafter{\the\@temptokena\null\partial{#1}^{#2}}%
	\else
	  \advance\@tempcnta by \@ne
	  \@temptokena\expandafter{\the\@temptokena\null\partial#1#2}
	\fi
    \fi
}
\makeatother

% inline partielle Ableitung als flacher Bruch
\makeatletter
\newcommand\fpder[2]{%
    \begingroup
    \@temptokena{\@gobble}%
    \@tempcnta\z@
    \@for\var:=#2\do{%
        \expandafter\@fpder\var\relax
    }%
    \ensuremath{{\partial
    \ifnum\@tempcnta>\@ne
        ^{\the\@tempcnta}%
    \fi
    #1}/{\the\@temptokena}}%
    \endgroup
}
\def\@fpder#1#2\relax{%
    \ifx\relax#2\relax
        \advance\@tempcnta by \@ne
        \@temptokena\expandafter{\the\@temptokena\null\partial{#1}}%
    \else
	\if!\ifnum9<1#2!\else_\fi%falls #2 eine Zahl ist...
	  \advance\@tempcnta by #2\relax
	  \@temptokena\expandafter{\the\@temptokena\null\partial{#1}^{#2}}%
	\else
	  \advance\@tempcnta by \@ne
	  \@temptokena\expandafter{\the\@temptokena\null\partial#1#2}
	\fi
    \fi
}
\makeatother

% inline partielle Ableitung
\makeatletter
\newcommand\ipder[2]{%
    \begingroup
    \@temptokena{\@gobble}%
    \@tempcnta\z@
    \@for\var:=#2\do{%
        \expandafter\@ipder\var\relax
    }%
    \ensuremath{\the\@temptokena #1}%
    \endgroup
}
\def\@ipder#1#2\relax{%
    \ifx\relax#2\relax
        \advance\@tempcnta by \@ne
        \@temptokena\expandafter{\the\@temptokena\null\partial_{#1}}%
    \else
	\if!\ifnum9<1#2!\else_\fi%falls #2 eine Zahl ist...
	  \advance\@tempcnta by #2\relax
	  \@temptokena\expandafter{\the\@temptokena\null\partial_{#1}^{#2}}%
	\else
	  \advance\@tempcnta by \@ne
	  \@temptokena\expandafter{\the\@temptokena\null\partial_{#1#2}}
	\fi
    \fi
}
\makeatother

